The Workshop on Internet Topology (WIT) Report

Internet topology analysis has recently experienced a surge of interest in computer science, physics, and the mathematical sciences. However, researchers from these different disciplines tend to approach the same problem from different angles. As a result, the field of Internet topology analysis and modeling must untangle sets of inconsistent findings, conflicting claims, and contradicting statements. On May 10-12, 2006, CAIDA hosted the Workshop on Internet topology (WIT). By bringing together a group of researchers spanning the areas of computer science, physics, and the mathematical sciences, the workshop aimed to improve communication across these scientific disciplines, enable interdisciplinary crossfertilization, identify commonalities in the different approaches, promote synergy where it exists, and utilize the richness that results from exploring similar problems from multiple perspectives. This report describes the findings of the workshop, outlines a set of relevant open research problems identified by participants, and concludes with recommendations that can benefit all scientific communities interested in Internet topology research.

==> Makefile <==
ROOT=report

TEXSRC=	$(ROOT).tex $(ROOT).bbl

all: $(ROOT).pdf

.SUFFIXES: .tex .dvi .ps .pdf

$(ROOT).dvi: $(TEXSRC)

MKPASS=@mkpass() { rm -f $(ROOT).dvi; $(MAKE) $(ROOT).dvi && touch $$*;}; mkpass

.pass1: $(TEXSRC) $(IMAGES)
	$(MKPASS) $@

.pass2: .pass1
	$(MKPASS) $@

$(ROOT).ps: .pass2

.tex.dvi:
	latex \\nonstopmode \\input{$<} || { rm $@; exit 1; }

.dvi.ps:
	dvips -t letter -Ppdf -G0 -o $@ $<

.ps.pdf:
	ps2pdf -dCompatibilityLevel=1.3 $<

clean:
	rm -f *.aux *.log *~
	rm -f .pass[123] .rebuild

realclean: clean
	rm -f *.ps *.dvi *.pdf *.sav *.bak
	chmod -x `find . -type f`

